Metric Registration of Curves and Surfaces using Optimal Control

This paper presents an overview of recent developments in the analysis of shapes such as curves and surfaces through Riemannian metrics. We show that several constructions of metrics on spaces of submanifolds can be unified through the prism of Riemannian submersions, with shape space metrics being induced from metrics defined on the top spaces. Computing the resulting Riemannian distances involves solving geodesic matching problems with boundary conditions. To deal efficiently with such variational problems, one can rely on an auxiliary family of "chordal" distances to simplify the treatment of boundary conditions, which we use to come up with a relaxed inexact formulation of the matching problem. This also allows to turn shape matching into optimal control problems and give a common framework to address them in practice. We then specify our analysis to the cases of intrinsic shape metrics defined using invariant Sobolev metrics on parametrized immersions, outer shape metrics induced from metrics on diffeomorphism groups of the ambient space and finally a recent hybrid model that combines those two approaches.

==> OptimalControl_old.tex <==
\section{Optimal control formulations of geodesic matching}

\todolaurent{I am a little unsure of how this section fits here or should rather be split and included in the next two sections. By suggesting an optimal control section at this stage, I think I had in mind a general introduction to optimal control, while the special cases for shape would be discussed in the relevant sections.}
Going back to the framework outlined in Section \ref{sec:submersion}, we can now derive more specifically the exact and relaxed formulations of the geodesic estimation problem given by \eqref{eq:r.sub.geod} and \eqref{eq:r.sub.geod.2} in the particular cases of the Riemannian submersions on shape spaces that will be of interest in the rest of this paper.

In the first situation, which will be treated in more details in Section \ref{sec:intrinsic_metrics}, we will consider the Riemannian submersion $\pi: \Imm(M,\R^d) \rightarrow \Imm(M,\R^d)/\Diff(M)$, with a Riemannian metric $G_{q}(\cdot,\cdot)$ on $\Imm(M,\R^d)$ invariant to the action of the reparametrization group $\Diff(M)$. We leave to Section \ref{sec:intrinsic_metrics} the technical construction of such metrics and in particular the question of the adequate regularity of the immersions but, at least formally for now, this setting is a particular instance of scenario (2) in the discussion of Section \ref{sec:submersion}. A geodesic between $b_0 = \pi(q_0)=[q_0]$ and $b_1 =\pi(q_1) = [q_1]$ minimizes $\int_0^1 G_{q(t)}(h(t),h(t)) dt$ subject to $\dot{q}(t) = h(t) \in T_{q(t)} \Imm(M,\R^d)$ and the boundary constraints $q(0) = q_0$ and $q(1) \in \pi^{-1}(b_1)$. The latter constraint can be replaced by jointly optimizing over variations in the fiber $q(1)\circ \tau$ for $\psi\in \Diff(M)$. In addition, as we shall see in the next section, $T_{q(t)} \Imm(M,\R^d)$ can be identified to the space of smooth vector fields in $C^{\infty}(M,\R^d)$, which leads to the following formulation of the exact geodesic matching problem:  
\begin{equation}
\label{eq:exactmathcing_intrinsic}
    \min_{h,\psi} \int_0^1 G_{q(t)}(h(t),h(t)) dt
\end{equation}
over $h \in L^2([0,1],C^{\infty}(M,\R^d))$, $\tau \in \Diff(M)$ with $q(0)=q_0$, $q(1)=q_1 \circ \tau$ and $\dot{q}(t) = h(t)$. Once again, it is often more practical to relax the end-time constraint using a fidelity term blind to fiber variations, in other words to reparametrizations of $q(1)$ and $q_1$. This is where the chordal distances defined in Section \ref{sec:chordal} fit in. In particular, using oriented varifold distances, the inexact matching problem may be formulated as:   
\begin{equation}
\label{eq:inexactmathcing_intrinsic}
    \min_{h} \int_0^1 G_{q(t)}(h(t),h(t)) \ dt + \lambda d^{\text{Var}}(q(1),q_1)^2
\end{equation}
with $\dot{q}(t) = h(t)$, $q(0)=q_0$ and $\lambda>0$ being a weight parameter. Interestingly, \eqref{eq:inexactmathcing_intrinsic} turns into an infinite-dimensional \textit{optimal control} problem (of Mayer-Lagrange type) in which, at each time $t$, the state of the system is the immersion $q(t)$ and the control is the vector field $h(t)$.

Let's consider now the second case study, which shall be developed in Section \ref{sec:LDDMM}, of a submersion from an outer deformation group acting on shapes. We will be interested in subgroups $G$ of the group $\Diff(\R^d)$ of diffeomorphisms of the ambient space $\R^d$ acting on any $[q] \in \Imm(M,\R^d)/\Diff(M)$ as $\phi \cdot [q] = [\phi \circ q]$. We assume that a right-invariant metric is given on $G$ which is summed up by the metric on its Lie algebra $\| \cdot \|_{\mf g}$ (the more precise construction of such groups and metrics is the subject of Section \ref{sec:LDDMM}). Following the discussion of case (1) in Section \ref{sec:submersion}, the geodesic between two shapes $b_0=[q_0]$ and $b_1=[q_1]$ is the result of the variational problem:
\begin{equation}
\label{eq:exactmathcing_outer}
    \min_{v} \int_0^1 \| v(t) \|_{\mf g}^2 \  dt .
\end{equation}
over $v \in L^2([0,1],\mf g)$, with $\dot{\varphi}(t) = v(t) \circ \varphi(t)$, $\varphi(0)=\text{id}$ and $[\varphi(1) \circ q_0] = [q_1]$. Equivalently, we can consider the dynamics directly on $q(t)=\varphi(t) \circ q_0$, as $\dot{q}(t) = v(t) \circ q(t)$ with the boundary constraint $[q(1)] = [q_1]$. The remaining issue is to deal with that constraint in the quotient space. As previously, this can be addressed by either optimizing over reparametrizations of $q_1$ or by considering the inexact matching equivalent of \eqref{eq:exactmathcing_outer} given by:
\begin{equation}
\label{eq:inexactmathcing_outer}
    \min_{v} \int_0^1 \| v(t) \|_{\mf g}^2 \  dt + \lambda d^{\text{Var}}(q(1),q_1)^2.
\end{equation}
where $q(0)=q_0$, $\dot{q}(t) = v(t) \circ q(t)$. We again end up with an optimal control problem similar to \eqref{eq:inexactmathcing_intrinsic}, although the control $v$ belongs here to a Lie algebra of vector fields defined on the full $\R^d$ with a metric $\|v\|_{\mf g}$ measuring its global regularity, while \eqref{eq:inexactmathcing_intrinsic} controls the evolution of $q$ through locally defined vector fields and metrics. As we will evidence in the following, this distinction leads to important differences in the properties of the respective geodesics and distances.  
